Just-in-Time Reconstruction: Inpainting Sparse Maps using Single View Depth Predictors as Priors

We present ``just-in-time reconstruction" as real-time image-guided inpainting of a map with arbitrary scale and sparsity to generate a fully dense depth map for the image. In particular, our goal is to inpaint a sparse map --- obtained from either a monocular visual SLAM system or a sparse sensor --- using a single-view depth prediction network as a virtual depth sensor. We adopt a fairly standard approach to data fusion, to produce a fused depth map by performing inference over a novel fully-connected Conditional Random Field (CRF) which is parameterized by the input depth maps and their pixel-wise confidence weights. Crucially, we obtain the confidence weights that parameterize the CRF model in a data-dependent manner via Convolutional Neural Networks (CNNs) which are trained to model the conditional depth error distributions given each source of input depth map and the associated RGB image. Our CRF model penalises absolute depth error in its nodes and pairwise scale-invariant depth error in its edges, and the confidence-based fusion minimizes the impact of outlier input depth values on the fused result. We demonstrate the flexibility of our method by real-time inpainting of ORB-SLAM, Kinect, and LIDAR depth maps acquired both indoors and outdoors at arbitrary scale and varied amount of irregular sparsity.

==> extras.tex <==
\begin{table*}
\caption{Comparison of the proposed method using different combination of confidence masks on the NYUv2 dataset.}
\centering
	\resizebox{\textwidth}{!}{ %
    	\begin{tabular}{ccccccccc}
        %\cline{2-6}
        \multicolumn{9}{l}{} \\ \toprule
        &  \multicolumn{2}{c}{RMSE} &\multicolumn{2}{c}{Relative Difference} & Scale Invariant Error & \multicolumn{3}{c}{Within $\delta$} \\
        \multicolumn{1}{c}{Method} & linear & log & Abs & Sqr& & $\delta$ & $\delta^2$ & $\delta^3$ \\ \midrule
                  Sparse Depth Points  & 2.838 & 4.558 &0.895& 2.349& 4.147& 46.7\% & 49.7\% & 52.5\% \\
          Delaunay Triangulated Sparse Depth  & 1.496 & 0.750 &0.373& 0.656& 0.513& 39.5\% & 66.3\% & 80.6\% \\
        Eigen \cite{Eigen2014} & 0.704 & 0.412 &0.168& 0.139& 0.083& 74.0\% & 94.8\% & 98.5\% \\
    	Ours (Equal Confidence)  & 0.691 & 0.410& 0.163 & 0.134& 0.081 & 75.0\% & 95.2\% & \textbf{98.7\%} \\ 
    	Ours (Learnt Net) &0.698 &0.410&0.163&0.137 & 0.081& 74.7\% & 95.2\% & \textbf{98.7\%} \\ 
        Ours (Learnt DT) & 0.686 &0.410&0.162& 0.133&0.080 &75.2\% & 95.2\% & \textbf{98.7\%} \\
	Ours (Learnt Net and DT) & \textbf{0.681} & \textbf{0.408}&\textbf{0.161}&\textbf{0.131} & \textbf{0.079} & \textbf{75.5\%} & \textbf{95.4\%} & \textbf{98.7\%} \\ 
        \\

    	\end{tabular}
    }
\vspace{-1em}
\label{tab:NYU_preds_old}
\end{table*}
% \section{Background} 

% %\textcolor{blue}{This need to go away} this section we summarize the related literature to our paper which in turn inspired the ideas presented in this work. First, we present depth estimation techniques from RGB images followed by the methods of fusing multiple modes to obtain a refined depth map. Finally, we look at techniques of learning a confidence map given an input and its corresponding ground truth.

% \textcolor{blue}{Structure of literature review if needed mostly used in intro already:}

% %\textbf{Visual SLAM}(gives a large scale map which contains fused information from multiple-view, computed uncertainties,is suited for storage, is well studied and is immensely useful for localization of the bot, but might be at a scale, is very sparse.).

% %\textbf{CNNs for Geometry}: (CNNs allows to capture relationships between the image and the depth and have much richer understanding about the distributions of valid partial maps, relates RGB observations to depths directly, most approaches at test time use one or few images, not straight forward to extend to multiple views, difficult to fuse with other sensory data, is No association with the stored maps which we use for localization.

% %\textbf{Uncertainty estimation and CNN}:% using CNN as virtual depth sensors.

% %\textbf{Data Fusion:}% works well for sensors capturing the data at the same resolution, does not cope with scale changes, how do you fuse sparse and dense data?
% %\textbf{Inpainting baselines} learned?/non-learned
% %\textbf{Misc}%Stuff which is vaguely related like posenet and need to be cited

% %\textcolor{blue}{consider removed}Reconstructing the 3D geometry of a scene is a well studied vision problem. Some of the early approaches revolved around creating a sparse representation of the world \cite{ORBSLAM_2015,Klein2007} with adequate information to track the robot location. With advances in computational power SLAM systems capable of generating denser point cloud \cite{Engel2014,Newcombe2011} became a popular choice. However, sparse SLAM systems are still commonly used when the deploy environment has limited on board computational complexity (e.g drones). In this work, we use the sparse depth maps created from \cite{ORBSLAM_2015} as one of the inputs in the fusion process. The other input being a depth map generated from a convolutional neural network given an RGB image \cite{Eigen2014,garg2016unsupervised,Depth2015Liu,laina2016deeper}. The resurgence of artificial neural networks has enabled a multitude of geometry based learning algorithms in which estimating depth from a monocular  image has been well received by the robotics and the vision community due to its close resemblance to structure from motion(SfM) and SLAM systems.

% \textcolor{blue}{dont know what is this about} As it was pointed out in \cite{Facil2016} by Facil et al. both neural net based single view depth estimation systems and SLAM system based multi-view depth estimation systems come with a number of caveats. More concretely, they showed that there are large errors in high gradient regions compared to low gradient regions in neural net based systems while this relationship is inverted for multi-view systems. They proposed a non-rigid fusion algorithm to preserve the desirable features of both approaches. 
% %Fertsl et al. were able fuse depths captured from two different sensors \cite{Ferstl2013}. A time of flight tensor which  operates at a large frame rate although, with a low lateral resolution and high acquisition noise was combined with the output of a stereo sensor which has a relatively large lateral resolution. They employ a primal-dual optimization scheme to perform the fusion process. On a similar note \cite{Liu2015} Liu et al. were also able to fuse depths from IR based depth sensor and a stereo rig. However, the fundamental difference between the previous  approaches and ours is scale invariant and we use a CNN to predict the fusion weights for each modality enabling us to readily discard the outliers during runtime without further processing.

% \textcolor{blue}{para below should go mostly after the method section partially in the intro and partially in the experimental section}
% %To the best of our knowledge our work is the first to perform learnt confidence based depth fusion. Concurrently, \cite{Ummenhofer2016} also proposed to learn confidence of optical flow predictions and \cite{Tateno2017} proposed to propagate depth map predictions of a neural network using a hand calculated confidence map. We draw inspiration from the works of Eigen and Fergus \cite{Eigen2014} as well as Krahenbuhl et al. \cite{Krahenbuhl2012}. Eigen et al. were primarily focused on learning depths from a single image and did not model the fusion of multiple depth maps. However, in their training loss function they employed a a scale-invariant term which allowed them to overcome the global scale ambiguity of the scene. We also employ a scale-invariant term precisely for the same reason which is more desirable in our case as the quantities we fuse are in significantly different scales. Krahenbuhl et al. \cite{Krahenbuhl2012} defined a fully connected CRF model parameterized by the distance and color intensities of the pixels using a linear combination of two Gaussian kernels to improve semantic segmentation. Our model on the other hand has as many learnable parameters as the number of pixels in all of the input depth maps capturing all information in the input depth maps while taking into account their pixelwise confidences.

% Our Fully Connected CRF formulation has (i) more flexibility than a Gaussian Fully Connected CRF and can be used for probabilistic fusion of sparse/dense signals (not limited to depth) coming at different scales and (ii) is having similar time complexity of inference as the fully connected Gaussian CRFs. In a Gaussian CRF pairwise connectivity weights are restricted and defined by the global mean and variance of the Gaussian-RBF kernel. Our formulation is not composed of Gaussian RBF kernels and therefore high dimensional filtering approximations [14] or local approximations based on kernel variance do not apply and yet still not needed in our case for fast inference of our fully connected pairwise terms, which also saves some processing overhead. Our model is more flexible in the sense that it only relies on a simple yet intuitive relaxation of our pairwise weight $c_{ij}^{(m)}=c_i^{(m)}c_j^{(m)}$ for fast inference, which implies that the confidence of the pairwise term is as good as the product of the individual confidences of the depths forming the pairwise constraint. This formulation also allows our model to handle depth maps with arbitrary sparsity structure, and the pairwise terms are scale invariant by design. As a side contribution we also propose a way to learn the confidences of the noisy/arbitrary scale depth maps given groundtruth (e.g. Kinect) depth and RGB image. The training loss for learning per-pixel confidences is based on the same fully connected CRF energy that is proposed for inference, and bear O(N) time complexity for computing gradients during backpropagation. For sparse signals like ORBSLAM performing delaunay triangulation on the sparse depth map before passing to the network allowed significant speed up in training, a smaller network capacity, and overall better confidence map predictions for the sparse depth map (after binary masking the prediction).




% \section{THIS IS DUMPED AS OLD EXPLAINATION OF FULLY CONNECTED TERM}
% \textcolor{red}{Rephrased and written above}
% By minimizing $E_{fc}$, $y$ is forced to satisfy all possible pairwise log depth relationships in $y^d$ weighted by the pairwise confidence weights $c_{ij}^d, \forall (i,j)$. In order to better understand the scale-invariant property, we can re-write the pairwise expression in \eqref{energy_fc} as $(ln(d_j/d_i) - ln(d_j^d/d_i^d)^2$ where $d_i$ and $d_j$ are the corresponding depth values of $y_i$ and $y_j$. Since depth ratio is independent of depth scale, \eqref{energy_fc} would be minimized even if $y$ and $y^d$ are at different scales provided their pairwise depth relationships are consistent. Therefore $E_{fc}$ is primarily important for extracting information out of input depth maps that are at a different scale to the sparse map.

% \textcolor{red}{Read above and edit above} a crucial step, we approximate $c_{ij}^d = c_i^dc_j^d$. This simple approximation significantly reduces the number of parameters to  learn as well as allow for tractable inference (refer section \ref{inference}). Intuitively the approximation implies that the confidence of the pairwise term is as good as the product of the individual confidences of $c_i^d$ and $c_j^d$ forming each pairwise loss. Note that our definition of $c_{ij}^d$ also enables $E_{fc}$ to operate on any $y^d$ with arbitrary sparsity structure. In that case the normalizer N should be replaced with the number of valid points in $y^d$. In our case however $y^d$ is dense. With the definition of $c_{ij}^d$, equation \eqref{energy_fc} can be written in an alternate form that allows for linear time computation of the fully connected term which is helpful during inference (refer section \ref{inference}):
% \begin{equation} 
% \label{energy_fc_lt}
% \begin{aligned}
% E_{fc}(y) &= \frac{1}{N} \textstyle{\sum}_j^N c_j^d \displaystyle \sum_i^N  c_i^d (y_i - y_i^d)^2 \\ &- \frac{1}{N} \Big(\sum_i^N c_i^d (y_i - y_i^d)\Big)^2 \\
% \end{aligned}
% \end{equation}


==> old_equations.tex <==
% \subsection{Inference Loss Function}
%Similar to \cite{Eigen2014}, our inference loss function operates on (natural) log depths as it allows writing depth ratios as differences, and makes it easier to define a unary term, as discussed further below. The output after inference is a fused and refined log depth map which we denote as $\mathbf{y} = [y_1, .., y_N] = ln(\mathbf{d}) = [ln(d_1), .., ln(d_N)]$, where $\mathbf{d}$ is the refined depth map and $N$ is the number of pixels in the image. The input log depth maps are denoted by $\mathbf{y}^{(m)} = [y_1^{(m)}, .., y_N^{(m)}], m = 1...M$, and their respective confidence maps are denoted by $\mathbf{c}^{(m)}=[c_1^{(m)}, .., c_N^{(m)}], m = 1...M$, where $M$ is the number of input log depth maps. For simplicity we assume all depth maps are aligned in the same coordinate frame. We construct the following energy which we minimize with respect to $\mathbf{y}$:
%
%\begin{equation} 
%\label{energy_inference_highlevel}
%\begin{aligned}
% E(\mathbf{y}) = &\sum_m^M E^{(m)}(\mathbf{y}) \\
%\end{aligned}
%\end{equation}
%where,
%\begin{equation} 
%\label{energy_inference}
%\begin{aligned}
% E^{(m)}(\mathbf{y}) = \alpha_u^{(m)} E_u^{(m)}%(\mathbf{y}) + \beta^{(m)} E_{fc}^{(m)}(\mathbf{y}) + \gamma^{(m)} E_{lc}^{(m)}(\mathbf{y}) \\
%\end{aligned}
%\end{equation}

%In \eqref{energy_inference}, $E_{u}^{(m)}$ is the unary term, $E_{fc}^{(m)}$ is the fully-connected pairwise term and $E_{lc}^{(m)}$ is the locally connected pairwise term. The first term penalizes absolute log depth error and thus influences the final scale of $\mathbf{y}$, while the latter two terms penalize incorrect pairwise log depth relationships and are scale-invariant measures. The tunable parameters $\alpha_u^{(m)}>0$, $\beta^{(m)}>0$, and $\gamma^{(m)}>0$ control the importance of each term for each log depth map $m$.

% We begin by defining $E_{fc}^{(m)}$ as follows:
% \begin{equation} 
% \label{energy_fc}
% \begin{aligned}
% E_{fc}^{(m)}(\mathbf{y}) = \frac{1}{2N_v^{(m)}}\sum_{i,j} c_{ij}^{(m)} \big((y_j - y_i ) - (y_j^{(m)} - y_i^{(m)})\big)^2 \\
% \end{aligned}
% \end{equation}
% where $N_v^{(m)}$ is the total number of valid pixels in log depth map $m$. By minimizing $E_{fc}^{(m)}(\mathbf{y})$, $\mathbf{y}$ is forced to satisfy all possible pairwise log depth relationships in $\mathbf{y}^{(m)}$ weighted by the pairwise confidence weights $c_{ij}^{(m)}, \forall (i,j)$, where $0 \leq c_{ij}^{(m)} \leq 1$. In order to better understand the scale-invariant property, we can re-write the pairwise expression in \eqref{energy_fc} as $(ln(d_j/d_i) - ln(d_j^{(m)}/d_i^{(m)}))^2$ where $d_i$ and $d_j$ are the corresponding depth values of $y_i$ and $y_j$. Since depth ratio is independent of depth scale, \eqref{energy_fc} would be minimized even if $\mathbf{y}$ and $\mathbf{y}^{(m)}$ are at different scales provided their pairwise depth relationships are consistent. Therefore $E_{fc}^{(m)}$ is primarily important for extracting information out of input depth maps $\mathbf{y}^{(m)}$ that are at a random unknown scale (Figure \ref{fig:fusions}). The normalization by $N_v^{(m)}$ is necessary as a depth map with more valid pixels will bear a larger cost per pixel than a sparser one, and hence the normalization reduces this bias.

% In a crucial step, we approximate $c_{ij}^{(m)} = c_i^{(m)}c_j^{(m)}$, where $0 \leq c_i^{(m)} \leq 1, \forall {i}$. Doing so significantly reduces the number of parameters to be learnt as well as allow \eqref{energy_fc} to be written in a form that allows for linear time computation as shown below. Intuitively the approximation implies that the confidence of the pairwise term is as good as the product of the individual confidences of $c_i^{(m)}$ and $c_j^{(m)}$ forming each pairwise loss. The confidence weight for a pixel in $\mathbf{y}^{(m)}$ is defined as $c_i^{(m)}=b_i^{(m)}\hat{c}_i^{(m)}$, where $\mathbf{b}^{(m)}=[b_1^{(m)},...,b_N^{(m)}]$ is a known binary mask with $1$s representing valid pixels in $\mathbf{y}^{(m)}$, and $\hat{\mathbf{c}}^{(m)}=[\hat{c}_1^{(m)},...,\hat{c}_N^{(m)}]$ is the confidence map for $\mathbf{y}^{(m)}$ which we will learn to predict (section \ref{learning}). Note that $\hat{\mathbf{c}}^{(m)}$ can also be deduced from some external confidence measurement source if available.

% Equation \eqref{energy_fc} can now be re-written in a linear-time computation form as follows:
% \begin{equation} 
% \label{energy_fc_lt}
% \begin{aligned}
% E_{fc}^{(m)}(\mathbf{y}) &= \frac{1}{N_v^{(m)}} \textstyle{\sum}_j^N c_j^{(m)} \displaystyle \sum_i^N  c_i^{(m)} (y_i - y_i^{(m)})^2 \\ &- \frac{1}{N_v^{(m)}} \Big(\sum_i^N c_i^{(m)} (y_i - y_i^{(m)})\Big)^2 \\
% \end{aligned}
% \end{equation}
 
% The first term of \eqref{energy_fc_lt} resembles a unary term and provides a basis for defining $E_u^{(m)}$:
% \begin{equation} 
% \label{energy_unary}
% \begin{aligned}
% E_u^{(m)}(\mathbf{y}) = \frac{1}{N_v^{(m)}}\textstyle{\sum}_j^N \displaystyle c_j^{(m)}\sum_i^N  c_i^{(m)} (y_i - y_i^{(m)})^2 \\
% \end{aligned}
% \end{equation}

% Finally $E_{lc}^{(m)}$ penalizes inconsistency in pairwise depth relationships in a local neighborhood around each pixel $i$. This term is helpful for extracting information out of depth maps with a lot of global errors but fewer local ones. While the neighborhood size can be arbitrary, a neighbourhood that is too large can make the solution increasingly biased towards a particular $\mathbf{y}^{(m)}$. 
% The end-effect is similar to local smoothing carried out in most image denoising methods, but ours is also data-driven. $E_{lc}^{(m)}$ is most important for instance when fusing a sparse depth map $\mathbf{y}^{(1)}$ with a dense depth map $\mathbf{y}^{(2)}$, where we can increase the tunable weight $\gamma^{(2)}$ corresponding to $E_{lc}^{(2)}$ so that $\mathbf{y}^{(2)}$'s depth values can be used to  ''smooth over'' the areas where the sparse depths points are fused, which are otherwise slightly prominent in the fused result (Figure \ref{fig:fusions}). For computational efficiency we only consider a 4-connected graph and we will refer to the set of 4 pixels neighboring $i$ as $\mathcal{N}(i)$. $E_{lc}^{(m)}$ is defined as:
% \begin{equation} 
% \label{energy_lc}
% \begin{aligned}
% E_{lc}^{(m)}(\mathbf{y}) = \sum_{i,k} c_i^{(m)}c_k^{(m)} \big((y_k - y_i ) - (y_k^{(m)} - y_i^{(m)})\big)^2 \\
% \end{aligned}
% \end{equation}

% where $k\in{\{+u(i),+v(i)\}}$ denotes pixel locations to the right and bottom of pixel $i$ in the image plane. Note that in effect we are repeating some of the terms already present in $E_{fc}^{(m)}$. For added flexibility in the neighborhood size leading to potential improvement in the fusion result, $E_{lc}^{(m)}$ can be modified as a fully connected term multiplied with a pixel-distance based Gaussian RBF-kernel similar to \cite{Campbell2013}\cite{SURGE}, but at the cost of added computational complexity.

% Combining \eqref{energy_unary}, \eqref{energy_fc_lt}, and \eqref{energy_lc} into \eqref{energy_inference} we obtain:

% \begin{equation} 
% \label{energy_inference_long}
% \begin{aligned}
% E^{(m)}(\mathbf{y}) = & \frac{\alpha^{(m)}}{N_v^{(m)}}  \textstyle{\sum}_j^N \displaystyle c_j^{(m)} \sum_i^N  c_i^{(m)}(y_i - y_i^{(m)})^2 \\ 
% -& \frac{\beta^{(m)}}{N_v^{(m)}} \Big(\sum_i^N c_i^{(m)} (y_i - y_i^{(m)})\Big)^2 \\
% +&\gamma^{(m)} \sum_{i,k} c_i^{(m)}c_k^{(m)} \big((y_k - y_i ) - (y_k^{(m)} - y_i^{(m)})\big)^2 \\
% \end{aligned}
% \end{equation}
% where $\alpha^{(m)} = \alpha_u^{(m)} + \beta^{(m)}$ and therefore $\alpha^{(m)} \geq \beta^{(m)}$.
